TIMBER: On supporting data pipelines in Mobile Cloud Environments

The radical advances in mobile computing, the IoT technological evolution along with cyberphysical components (e.g., sensors, actuators, control centers) have led to the development of smart city applications that generate raw or pre-processed data, enabling workflows involving the city to better sense the urban environment and support citizens' everyday lives. Recently, a new era of Mobile Edge Cloud (MEC) infrastructures has emerged to support smart city applications that aim to address the challenges raised due to the spatio-temporal dynamics of the urban crowd as well as bring scalability and on-demand computing capacity to urban system applications for timely response. In these, resource capabilities are distributed at the edge of the network and in close proximity to end-users, making it possible to perform computation and data processing at the network edge. However, there are important challenges related to real-time execution, not only due to the highly dynamic and transient crowd, the bursty and highly unpredictable amount of requests but also due to the resource constraints imposed by the Mobile Edge Cloud environment. In this paper, we present TIMBER, our framework for efficiently supporting mobile daTa processing pIpelines in MoBile cloud EnviRonments that effectively addresses the aforementioned challenges. Our detailed experimental results illustrate that our approach can reduce the operating costs by 66.245% on average and achieve up to 96.4% similar throughput performance for agnostic workloads.

==> serverless.tex <==
\subsection{Containers}
We can describe each application as a set of functions that run inside Docker containers. Each function can be replicated in many containers that run in parallel. For each function replica $r_i$ we allocate $m$ MBs of memory and $c$ CPUs. The containers are homogeneous, that means that all of the containers have the same CPU and memory allocation. The total allocated CPUs and memory for one function is the sum of the CPUs and memory that are allocated per replica. 

The container allocation cannot exceed the resources of a single node in the cluster. In this case the container will not be scheduled by the Orchestrator.

A process called Watchdog runs in every container and receives function invocation calls as HTTP Post requests. When it receives a request, it creates a new process that runs the function code and dispaches the request to that process. Then it responds with the standard output of that process to the initial request. A more recent version of Watchdog, called Of-Watchdog keeps the function process warm between invocations in contrast with the classic watchdog, that forks one process per request. In this way it achieves higher throughput and enables re-use of expensive resources such as database connection pools or machine-learning models.
